Word-Graph2vec: An efficient word embedding approach on word co-occurrence graph using random walk technique

Word embedding has become ubiquitous and is widely used in various natural language processing (NLP) tasks, such as web retrieval, web semantic analysis, and machine translation, and so on. Unfortunately, training the word embedding in a relatively large corpus is prohibitively expensive. We propose a graph-based word embedding algorithm, called Word-Graph2vec, which converts the large corpus into a word co-occurrence graph, then takes the word sequence samples from this graph by randomly traveling and trains the word embedding on this sampling corpus in the end. We posit that because of the limited vocabulary, huge idioms, and fixed expressions in English, the size and density of the word co-occurrence graph change slightly with the increase in the training corpus. So that Word-Graph2vec has stable runtime on the large-scale data set, and its performance advantage becomes more and more obvious with the growth of the training corpus. Extensive experiments conducted on real-world datasets show that the proposed algorithm outperforms traditional Word2vec four to five times in terms of efficiency and two to three times than FastText, while the error generated by the random walk technique is small.

==> sections/problem_formulation.tex <==
\section{Problem Formulation}
\label{sec:problem_formulation}





The task of this paper is to propose a method that can efficiently learn high-quality word embedding from a large-scale corpus. The word co-occurrence graph, whose each node is a word, whose edges represent co-occurrences between the word and its adjacency node, and whose edge direction represents word order, is extracted from the large-scale corpus. Then, our task maps all words (word and node is one-to-one correspondence) in the graph to a low-dimensional embedding space, in which each word is represented as a dense embedding space. The local relationship and deep connection among words have semantic connections in the embedding space. Formally, the problem can be defined as:

\noindent \textbf{Input}: a preprocessed monolingual corpus with billions of words and with hundreds of thousands of words in the vocabulary.

\noindent \textbf{Output}: a global representation matrix $\Phi \in \mathbb{R}^{|V| \times d} $, whose $\Phi_{i}$ ($ i\mbox{-}th $ row) is a $ d\mbox{-}dimensional $ vector representing the word $ \mathcal{V}_{i} $.

The word co-occurrence graph is defined as follows. Let $G = (V, E)$ be a directed weighted word graph, where $V$ represents the set of nodes, and $ E \subseteq V_{i} \times V_{j} $ defines the edges between nodes. As shown in Figure \ref{fig:graph_sample}, each edge has a non-negative weight $ W_{ij} $, which is used to describe the strength among the connecting nodes; If two nodes are disconnected, the edge weight $ W_{ij} $ is set to zero. Therefore, a matrix $ W = \left[ W_{ij}\right] \in \mathbb{R}^{|V| \times |V|} $  is used to represent all weights between nodes, and a vector $PW = \left[ PW_{i}\right] \in \mathbb{R}^{1 \times |V|} $ is represented as the weights on each nodes. Figure~\ref{fig:graph_sample} shows an example of word co-occurrence graph, which contains four words (a, b, c, and d). 

%In addition, all the other notations in our paper are listed in Table~\ref{tab:symbols}
%
%\begin{table}
%	\caption{Symbols}
%	\label{tab:symbols}
%	\resizebox{\linewidth}{!}{
	%		\begin{tabular}{|c|l|}
		%			\hline
		%			\textbf{Symbol} & \textbf{Definition}\\ \hline
		%			$ G $ & The directed and  weighted word graph \\ \hline
		%			$ N $ & The set of corpus \\ \hline
		%			$ |N| $ & The size of corpus \\ \hline 
		%			$ |\mathrm{V}| $ & The number of nodes(words) \\ \hline
		%			$ V $ & The set of nodes\\ \hline
		%			$ |\mathrm{V}| $ & The number of nodes(words) \\ \hline
		%			$ E $ & The edge set \\ \hline
		%			$ |\mathrm{E}| $ & The number of edges \\ \hline
		%			$ \mathcal{V} $ & The vocabulary of corpus; Noted that the word and the node is one-to-one correspondence. \\ \hline
		%			$ W $ & The weighted adjacency matrix $W \in \mathbb{R}^{|V| \times |V|} $of nodes \\ \hline
		%			$ \Phi $ & The global representation matrix $\Phi \in \mathbb{R}^{|V| \times d} $, whose $ i\mbox{-}th $ row $\Phi_{i}$ is a $ d\mbox{-}dimensional $ vector representing the word $ \mathcal{V}_{i} $\\ \hline
		%			$ Outdeg_{(u)} $ & Out-degree of node $ u $ \\ \hline
		%			$ TF_{(v,d)} $ &  The frequency of word $ v \in \mathcal{V} $ in document $ d $ \\ \hline
		%			$ IDF_{(v)} $ &  The inverse text frequency of word $ v \in \mathcal{V} $ \\ \hline
		%			$ TF\mbox{-}IDF_{(v)} $ &  The tf-idf value of word $ v \in \mathcal{V} $ \\ \hline
		%			$ n_{v,d} $ & The number of occurrences of the word $ v \in \mathcal{V} $ in document $ d $\\ \hline
		%			$ \sum_{k} n_{k, d} $ & The sum of the occurrences of all words in the document $ d $\\ \hline
		%			$ PW_{u} $ & Probability of word occurrence of node $ u $ \\ \hline
		%			$ \pi_{vx} $ & The non normalized transition probability between nodes $ v $ and $ x $ \\ \hline
		%			$p$ & The probability parameter that controls the return from node $ v $ to starting node $ t $ in sampling\\ \hline
		%			$q$ & Probability parameter of control node $ v $ accessing new node in sampling\\ \hline
		%			$\alpha_{pq}$ &  The state transition equation \\ \hline
		%			$d_{tx}$ & The shortest path distance between nodes $ t $ and $ x $ \\ \hline
		%			$l \, \& \, walk\_length$ &  The number of node will be involved in each random walk \\ \hline	
		%			$c$ &  The sampling sequence with length $ l $ \\ \hline	
		%			$Ns(c_{j}) $ & The neighborhood word set with $ c_{i} $ as the center and $ k $ as the window size \\ \hline
		%			$Z$ &  The normalizing constant \\ \hline	
		%			$ R_{u} $ & Traversal times of each node as the starting node of node $ u $ \\ \hline		
		%			$ average\_walks $ & The basic value of the given number of walks per node \\ \hline
		%			$ |\mathrm{C}| $ &  The total number of document in the corpus \\ \hline
		%			$ {P}(Ns(u) \mid f(u)) $	& The conditional probability of words’ co-occurrence in the neighborhood \\ \hline
		%			$ {P}(n_{i} \mid f(u)) $	& Softmax function used to approximate the probability distribution for each node $ n_{i} $\\ \hline
		%		\end{tabular}
	%	}
%\end{table}


\begin{figure}
	\begin{minipage}{0.48\linewidth}
		\centerline{\includegraphics[width=4.0cm]{figures/graph_sample.png}}
	\end{minipage}
	\hfill
	\begin{minipage}{.48\linewidth}
		$$
		W =\left(\begin{array}{llll}
			0 & 3 & 0 & 1 \\
			0 & 5 & 0 & 0 \\
			0 & 2 & 0 & 7 \\
			3 & 1 & 0 & 0
		\end{array}\right)
		$$
		$$
		PW =\left ( 
		\begin{array}{llll}
			0.182 \\ 
			0.228 \\ 
			0.409 \\
			0.182 \\
		\end{array}\right )
		$$
	\end{minipage}
	\caption{An example of the directed weighted graph $G$, adjacency matrix $W$ and the node's weight vector $PW$.}
	\label{fig:graph_sample}
\end{figure}

%Yuanzhe: Is the score on Figure 1 correct? Please make sure!


